Energy resolution and linearity of XENON1T in the MeV energy range

Xenon dual-phase time projection chambers designed to search for Weakly Interacting Massive Particles have so far shown a relative energy resolution which degrades with energy above $\sim$200 keV due to the saturation effects. This has limited their sensitivity in the search for rare events like the neutrinoless double-beta decay of $^{136}$Xe at its $Q$-value, $Q_{\beta\beta}\simeq$ 2.46 MeV. For the XENON1T dual-phase time projection chamber, we demonstrate that the relative energy resolution at 1 $\sigma/\mu$ is as low as (0.80$\pm$0.02) % in its one-ton fiducial mass, and for single-site interactions at $Q_{\beta\beta}$. We also present a new signal correction method to rectify the saturation effects of the signal readout system, resulting in more accurate position reconstruction and indirectly improving the energy resolution. The very good result achieved in XENON1T opens up new windows for the xenon dual-phase dark matter detectors to simultaneously search for other rare events.

==> Authors.tex <==
\author{E.~Aprile\thanksref{addr1}
        \and
        J.~Aalbers\thanksref{addr2}
        \and
        F.~Agostini\thanksref{addr3}
        \and
        M.~Alfonsi\thanksref{addr4}
        \and
        L.~Althueser\thanksref{addr5}
        \and
        F.~D.~Amaro\thanksref{addr6} % left Dec 2019
        \and
        V.~C.~Antochi\thanksref{addr2}
        \and
        E.~Angelino\thanksref{addr7}
        \and
        J.~Angevaare\thanksref{addr11} % !!!!!  NEW !!!!!
        \and
        F.~Arneodo\thanksref{addr8}
        \and
        D.~Barge\thanksref{addr2} % left Sep 2019
        \and
        L.~Baudis\thanksref{addr9}
        \and
        B.~Bauermeister\thanksref{addr2} % left Nov 2019
        \and
        L.~Bellagamba\thanksref{addr3}   % !!!!!  NEW !!!!!
        \and
        M.~L.~Benabderrahmane\thanksref{addr8}
        \and
        T.~Berger\thanksref{addr10} % left Jun 2019
        \and
        P.~A.~Breur\thanksref{addr11} % left Apr 2019
        \and
        A.~Brown\thanksref{addr9}
        \and
        E.~Brown\thanksref{addr10}
        \and
        S.~Bruenner\thanksref{addr11,addr12} % !!!!!  NEW second affiliation !!!!!
        \and
        G.~Bruno\thanksref{addr8}
        \and
        R.~Budnik\thanksref{addr13,also1} % !!!!!  NEW also at affiliation !!!!!
        \and
        C.~Capelli\thanksref{addr9,e1}
        \and
        J.~M.~R.~Cardoso\thanksref{addr6}
        \and
        D.~Cichon\thanksref{addr12}
        \and
        B.~Cimmino\thanksref{addr14} % !!!!!  NEW !!!!!
        \and
        M.~Clark\thanksref{addr23} % !!!!!  NEW !!!!!
        \and
        D.~Coderre\thanksref{addr15} % left Dec 2019
        \and
        A.~P.~Colijn\thanksref{addr11,also2}
        \and
        J.~Conrad\thanksref{addr2}
        \and
        J.~P.~Cussonneau\thanksref{addr16}
        \and
        M.~P.~Decowski\thanksref{addr11}
        \and
        A.~Depoian\thanksref{addr23}
        \and
        P.~Di~Gangi\thanksref{addr3}
        \and
        A.~Di~Giovanni\thanksref{addr8}
        \and
        R.~Di Stefano\thanksref{addr14} % !!!!!  NEW !!!!!
        \and
        S.~Diglio\thanksref{addr16}
        \and
        A.~Elykov\thanksref{addr15}
        \and
        G.~Eurin\thanksref{addr12} % left Aug 2019
        \and
        A.~D.~Ferella\thanksref{addr17,addr18} % !!!!!  NEW affiliation !!!!!
        \and
        W.~Fulgione\thanksref{addr7,addr18}
        \and
        P.~Gaemers\thanksref{addr11}
        \and
        R.~Gaior\thanksref{addr19} % !!!!!  NEW !!!!!
        \and
        A.~Gallo Rosso\thanksref{addr18} % left Mar 2019
        \and
        M.~Galloway\thanksref{addr9}
        \and
        F.~Gao\thanksref{addr1}
        \and
        M.~Garbini\thanksref{addr3} % left Mar 2019
        \and
        L.~Grandi\thanksref{addr20}
        \and
        C.~Hasterok\thanksref{addr12} % left Jul 2019
        \and
        C.~Hils\thanksref{addr4}
        \and
        K.~Hiraide\thanksref{addr21} % !!!!!  NEW JP!!!!!
        \and
        L.~Hoetzsch\thanksref{addr12} % !!!!!  NEW !!!!!
        \and
        E.~Hogenbirk\thanksref{addr11} % left Apr 2019
        \and
        J.~Howlett\thanksref{addr1}
        \and
        M.~Iacovacci\thanksref{addr14}
        \and
        Y.~Itow\thanksref{addr22,also3}% !!!!!  NEW JP!!!!! NEEDS to be confirmed!!!!!!!!!!
        \and
        F.~Joerg\thanksref{addr12}
        \and
        N.~Kato\thanksref{addr21} % !!!!!  NEW JP!!!!!
        \and
        S.~Kazama\thanksref{addr22}
        \and
        M.~Kobayashi\thanksref{addr1}
        \and
        G.~Koltman\thanksref{addr13}
        \and
        A.~Kopec\thanksref{addr23}
        \and
        H.~Landsman\thanksref{addr13}
        \and
        R.~F.~Lang\thanksref{addr23}
        \and
        L.~Levinson\thanksref{addr13}
        \and
        Q.~Lin\thanksref{addr1} % left Oct 2019
        \and
        S.~Lindemann\thanksref{addr15}
        \and
        M.~Lindner\thanksref{addr12}
        \and
        F.~Lombardi\thanksref{addr6}
        \and
        J.~A.~M.~Lopes\thanksref{addr6,also4}
        \and
        E.~L\'opez~Fune\thanksref{addr19}
        \and
        C. Macolino\thanksref{addr25}
        \and
        J.~Mahlstedt\thanksref{addr2}
        \and
        L.~Manenti\thanksref{addr8}  % !!!!!  NEW !!!!!
        \and
        A.~Manfredini\thanksref{addr9}
        \and
        F.~Marignetti\thanksref{addr14}
        \and
        T.~Marrod\'an~Undagoitia\thanksref{addr12}
        \and
        K.~Martens\thanksref{addr21} % !!!!!  NEW JP!!!!!
        \and
        J.~Masbou\thanksref{addr16}
        \and
        D.~Masson\thanksref{addr15}  %!!!!!  NEW back!!!!!
        \and
        S.~Mastroianni\thanksref{addr14}
        \and
        M.~Messina\thanksref{addr18}
        \and
        K.~Miuchi\thanksref{addr26} % !!!!!  NEW JP!!!!!
        \and
        A.~Molinario\thanksref{addr18}
        \and
        K.~Mor\aa\thanksref{addr1,addr2} % !!!!!  NEW affiliation !!!!!
        \and
        S.~Moriyama\thanksref{addr21}  %!!!!!  NEW JP!!!!!
        \and
        Y.~Mosbacher\thanksref{addr13}
        \and
        M.~Murra\thanksref{addr5}
        \and
        J.~Naganoma\thanksref{addr18}
        \and
        K.~Ni\thanksref{addr24}
        \and
        U.~Oberlack\thanksref{addr4}
        \and
        K.~Odgers\thanksref{addr10}
        \and
        J.~Palacio\thanksref{addr12,addr16} % !!!!!  NEW affiliation !!!!!
        \and
        B.~Pelssers\thanksref{addr2}
        \and
        R.~Peres\thanksref{addr9}
        \and
        J.~Pienaar\thanksref{addr20}
        \and
        V.~Pizzella\thanksref{addr12}
        \and
        G.~Plante\thanksref{addr1}
        \and
        J.~Qin\thanksref{addr23}
        \and
        H.~Qiu\thanksref{addr13} % left Jun 2019
        \and
        D.~Ram\'irez~Garc\'ia\thanksref{addr15}
        \and
        S.~Reichard\thanksref{addr9}
        \and
        A.~Rocchetti\thanksref{addr15}
        \and
        N.~Rupp\thanksref{addr12}
        \and
        J.~M.~F.~dos~Santos\thanksref{addr6}
        \and
        G.~Sartorelli\thanksref{addr3}
        \and
        N.~\v{S}ar\v{c}evi\'c\thanksref{addr15} % left Oct 2019
        \and
        M.~Scheibelhut\thanksref{addr4} % left Oct 2019
        \and
        S.~Schindler\thanksref{addr4} % left Mar 2019
        \and
        J.~Schreiner\thanksref{addr12}
        \and
        D.~Schulte\thanksref{addr5}
        \and
        M.~Schumann\thanksref{addr15}
        \and
        L.~Scotto~Lavina\thanksref{addr19}
        \and
        M.~Selvi\thanksref{addr3}
        \and
        F.~Semeria\thanksref{addr3} % !!!!!  NEW !!!!!
        \and
        P.~Shagin\thanksref{addr27}
        \and
        E.~Shockley\thanksref{addr20}
        \and
        M.~Silva\thanksref{addr6}
        \and
        H.~Simgen\thanksref{addr12}
        \and
        A.~Takeda\thanksref{addr21} % !!!!!  NEW JP!!!!!
        \and
        C.~Therreau\thanksref{addr16}
        \and
        D.~Thers\thanksref{addr16}
        \and
        F.~Toschi\thanksref{addr15}
        \and
        G.~Trinchero\thanksref{addr7}
        \and
        C.~Tunnell\thanksref{addr27}
        \and
        M.~Vargas\thanksref{addr5}
        \and
        G.~Volta\thanksref{addr9}
        \and
        O.~Wack\thanksref{addr12}  % left Mar 2019
        \and
        H.~Wang\thanksref{addr28} % left Jul 2019
        \and
        Y.~Wei\thanksref{addr24}
        \and
        C.~Weinheimer\thanksref{addr5}
        \and
        M.Weiss~Xu\thanksref{addr13}  % !!!!!  NEW !!!!!
        \and
        D.~Wenz\thanksref{addr4}
        \and
        C.~Wittweg\thanksref{addr5}
        \and
        J.~Wulf\thanksref{addr9} % left Mar 2019
        \and
        Z.~Xu\thanksref{addr1}  % !!!!!  NEW !!!!!
        \and
        M.~Yamashita\thanksref{addr21}  % !!!!!  NEW JP!!!!!
        \and
        J.~Ye\thanksref{addr24}
        \and
        G.~Zavattini\thanksref{addr3,also5}   % !!!!!  NEW !!!!!
        \and
        Y.~Zhang\thanksref{addr1}
        \and
        T.~Zhu\thanksref{addr1,e2}
        \and
        J.~P.~Zopounidis\thanksref{addr19}
        %\and
        (XENON Collaboration\thanksref{t1}).
}
%
%
\authorrunning{XENON Collaboration}
\thankstext{also1}{Also at \suny}
\thankstext{also2}{Also at \utrecht}
\thankstext{also3}{Also at \spacenagoya}
\thankstext{also4}{Also at \coimbrapoli}
\thankstext{also5}{At \ferrara}
\thankstext{e1}{\texttt{chiara.capelli@physik.uzh.ch}}
\thankstext{e2}{\texttt{tianyu.zhu@columbia.edu}}
\thankstext{t1}{\texttt{xenon@lngs.infn.it}}
%
%
\institute{\columbia\label{addr1} %1
        \and
        \stockholm\label{addr2} %2
        \and
        \bologna\label{addr3} %3
        \and
        \mainz\label{addr4} %4
        \and
        \munster\label{addr5} %5
        \and
        \coimbra\label{addr6} %6
        \and
        \torino\label{addr7} %7
        \and
        \nikhef\label{addr11} %11
        \and
        \nyuad\label{addr8} %8
        \and
        \zurich\label{addr9} %9
        \and
        \rpi\label{addr10} %10
        \and
        \heidelberg\label{addr12} %12
        \and
        \wis\label{addr13} %13
        \and
        \naples\label{addr14} %14
        \and
        \purdue\label{addr23} %23
        \and
        \freiburg\label{addr15} %15
        \and
        \subatech\label{addr16} %16
        \and
        \laquila\label{addr17} %17
        \and
        \lngs\label{addr18} %18
        \and
        \paris\label{addr19} %19
        \and
        \chicago\label{addr20} %20
        \and
        \tokyo\label{addr21} %21
        \and
        \nagoya\label{addr22} %22
        \and
        \ucsd\label{addr24} %24
        \and
        \lal\label{addr25} %25
        \and
        \kobe\label{addr26} %26
        \and
        \rice\label{addr27} %27
        \and
        \ucla\label{addr28} %28
}

==> authors_and_institutions.tex <==
\newcommand{\bologna}{\affiliation{Department of Physics and Astronomy, University of Bologna and INFN-Bologna, 40126 Bologna, Italy}}

\newcommand{\chicago}{\affiliation{Department of Physics \& Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}}

\newcommand{\coimbra}{\affiliation{LIBPhys, Department of Physics, University of Coimbra, 3004-516 Coimbra, Portugal}}

\newcommand{\columbia}{\affiliation{Physics Department, Columbia University, New York, NY 10027, USA}}

\newcommand{\lngs}{\affiliation{INFN-Laboratori Nazionali del Gran Sasso and Gran Sasso Science Institute, 67100 L'Aquila, Italy}}

\newcommand{\mainz}{\affiliation{Institut f\"ur Physik \& Exzellenzcluster PRISMA, Johannes Gutenberg-Universit\"at Mainz, 55099 Mainz, Germany}}

\newcommand{\heidelberg}{\affiliation{Max-Planck-Institut f\"ur Kernphysik, 69117 Heidelberg, Germany}}

\newcommand{\munster}{\affiliation{Institut f\"ur Kernphysik, Westf\"alische Wilhelms-Universit\"at M\"unster, 48149 M\"unster, Germany}}

\newcommand{\nikhef}{\affiliation{Nikhef and the University of Amsterdam, Science Park, 1098XG Amsterdam, Netherlands}}

\newcommand{\nyuad}{\affiliation{New York University Abu Dhabi, Abu Dhabi, United Arab Emirates}}

\newcommand{\purdue}{\affiliation{Department of Physics and Astronomy, Purdue University, West Lafayette, IN 47907, USA}}

\newcommand{\rpi}{\affiliation{Department of Physics, Applied Physics and Astronomy, Rensselaer Polytechnic Institute, Troy, NY 12180, USA}}

\newcommand{\rice}{\affiliation{Department of Physics and Astronomy, Rice University, Houston, TX 77005, USA}}

\newcommand{\stockholm}{\affiliation{Oskar Klein Centre, Department of Physics, Stockholm University, AlbaNova, Stockholm SE-10691, Sweden}}

\newcommand{\subatech}{\affiliation{SUBATECH, IMT Atlantique, CNRS/IN2P3, Universit\'e de Nantes, Nantes 44307, France}}

\newcommand{\torino}{\affiliation{INAF-Astrophysical Observatory of Torino, Department of Physics, University  of  Torino  and  INFN-Torino,  10125  Torino,  Italy}}

\newcommand{\ucla}{\affiliation{Physics \& Astronomy Department, University of California, Los Angeles, CA 90095, USA}}

\newcommand{\ucsd}{\affiliation{Department of Physics, University of California, San Diego, CA 92093, USA}}

\newcommand{\wis}{\affiliation{Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot 7610001, Israel}}

\newcommand{\zurich}{\affiliation{Physik-Institut, University of Zurich, 8057  Zurich, Switzerland}}

\newcommand{\paris}{\affiliation{LPNHE, Universit\'{e} Pierre et Marie Curie, Universit\'{e} Paris Diderot, CNRS/IN2P3, Paris 75252, France}}

\newcommand{\freiburg}{\affiliation{Physikalisches Institut, Universit\"at Freiburg, 79104 Freiburg, Germany}}

\newcommand{\lal}{\affiliation{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91405 Orsay, France}}

\newcommand{\naples}{\affiliation{Department of Physics ``Ettore Pancini'', University of Napoli and INFN-Napoli, 80126 Napoli, Italy}} 

\newcommand{\nagoya}{\affiliation{Kobayashi-Maskawa Institute for the Origin of Particles and the Universe, Nagoya University, Furo-cho, Chikusa-ku, Nagoya, Aichi 464-8602, Japan}}

\newcommand{\laquila}{\affiliation{Department of Physics and Chemistry, University of L'Aquila, 67100 L'Aquila, Italy}}

\newcommand{\tokyo}{\affiliation{Kamioka Observatory, Institute for Cosmic Ray Research, and Kavli Institute for the Physics and Mathematics of the Universe (WPI), the University of Tokyo, Higashi-Mozumi, Kamioka, Hida, Gifu 506-1205, Japan}}


\author{E.~Aprile}\columbia
\author{J.~Aalbers}\stockholm
\author{F.~Agostini}\bologna
\author{M.~Alfonsi}\mainz
\author{L.~Althueser}\munster
\author{F.~D.~Amaro}\coimbra % left Dec 2019
\author{V.~C.~Antochi}\stockholm
\author{E.~Angelino}\torino
\author{F.~Arneodo}\nyuad
\author{D.~Barge}\stockholm % left Sep 2019
\author{L.~Baudis}\zurich
\author{B.~Bauermeister}\stockholm % left Nov 2019
\author{L.~Bellagamba}\bologna   % !!!!!  NEW !!!!!
\author{M.~L.~Benabderrahmane}\nyuad
\author{T.~Berger}\rpi % left Jun 2019
\author{P.~A.~Breur}\nikhef % left Apr 2019
\author{A.~Brown}\zurich
\author{E.~Brown}\rpi
\author{S.~Bruenner}\nikhef\heidelberg % !!!!!  NEW second affiliation !!!!!
\author{G.~Bruno}\nyuad
\author{R.~Budnik}\altaffiliation[Also at ]{Simons Center for Geometry and Physics and C. N. Yang Institute for Theoretical Physics, SUNY, Stony Brook, NY, USA}\wis % !!!!!  NEW also at affiliation !!!!!
\author{C.~Capelli}\zurich
\author{J.~M.~R.~Cardoso}\coimbra
\author{D.~Cichon}\heidelberg
\author{B.~Cimmino}\naples % !!!!!  NEW !!!!!
\author{M.~Clark}\purdue % !!!!!  NEW !!!!!
\author{D.~Coderre}\freiburg % left Dec 2019
\author{A.~P.~Colijn}\altaffiliation[Also at ]{Institute for Subatomic Physics, Utrecht University, Utrecht, Netherlands}\nikhef
\author{J.~Conrad}\stockholm
\author{J.~P.~Cussonneau}\subatech
\author{M.~P.~Decowski}\nikhef
\author{A.~Depoian}\purdue
\author{P.~Di~Gangi}\bologna
\author{A.~Di~Giovanni}\nyuad
\author{R.~Di Stefano}\naples % !!!!!  NEW !!!!!
\author{S.~Diglio}\subatech
\author{A.~Elykov}\freiburg
\author{G.~Eurin}\heidelberg % left Aug 2019
\author{A.~D.~Ferella}\laquila\lngs % !!!!!  NEW affiliation !!!!!
\author{W.~Fulgione}\lngs\torino
\author{P.~Gaemers}\nikhef
\author{R.~Gaior}\paris % !!!!!  NEW !!!!!
\author{A.~Gallo Rosso}\lngs % left Mar 2019
\author{M.~Galloway}\zurich
\author{F.~Gao}\columbia
\author{M.~Garbini}\bologna % left Mar 2019
\author{L.~Grandi}\chicago
\author{C.~Hasterok}\heidelberg % left Jul 2019
\author{C.~Hils}\mainz
\author{K.~Hiraide}\tokyo % !!!!!  NEW JP!!!!!
\author{L.~Hoetzsch}\heidelberg % !!!!!  NEW !!!!!
\author{E.~Hogenbirk}\nikhef % left Apr 2019
\author{J.~Howlett}\columbia
\author{M.~Iacovacci}\naples
\author{Y.~Itow}\altaffiliation[Also at ]{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya, Aichi 464-8601, Japan} \nagoya     % !!!!!  NEW JP!!!!! NEEDS to be confirmed!!!!!!!!!!
\author{F.~Joerg}\heidelberg
\author{N.~Kato}\tokyo % !!!!!  NEW JP!!!!!
\author{S.~Kazama}\nagoya
\author{M.~Kobayashi}\columbia
\author{G.~Koltman}\wis
\author{A.~Kopec}\purdue
\author{H.~Landsman}\wis
\author{R.~F.~Lang}\purdue
\author{L.~Levinson}\wis
\author{Q.~Lin}\columbia % left Oct 2019
\author{S.~Lindemann}\freiburg
\author{M.~Lindner}\heidelberg
\author{F.~Lombardi}\coimbra\ucsd
\author{J.~A.~M.~Lopes}\altaffiliation[Also at ]{Coimbra Polytechnic - ISEC, Coimbra, Portugal}\coimbra
\author{E.~L\'opez~Fune}\paris
\author{C. Macolino}\lal
\author{J.~Mahlstedt}\stockholm
\author{L.~Manenti}\nyuad  % !!!!!  NEW !!!!!
\author{A.~Manfredini}\zurich
\author{F.~Marignetti}\naples
\author{T.~Marrod\'an~Undagoitia}\heidelberg
\author{K.~Martens}\tokyo % !!!!!  NEW JP!!!!!
\author{J.~Masbou}\subatech
\author{S.~Mastroianni}\naples
\author{M.~Messina}\lngs\nyuad
\author{K.~Miuchi}\kobe % !!!!!  NEW JP!!!!!
\author{A.~Molinario}\lngs
\author{K.~Mor\aa}\columbia\stockholm % !!!!!  NEW affiliation !!!!!
\author{S.~Moriyama}\tokyo  %!!!!!  NEW JP!!!!!
\author{Y.~Mosbacher}\wis
\author{M.~Murra}\munster
\author{J.~Naganoma}\lngs\rice
\author{K.~Ni}\ucsd
\author{U.~Oberlack}\mainz
\author{K.~Odgers}\rpi
\author{J.~Palacio}\subatech \heidelberg % !!!!!  NEW affiliation !!!!!
\author{B.~Pelssers}\stockholm
\author{R.~Peres}\zurich
\author{J.~Pienaar}\chicago
\author{V.~Pizzella}\heidelberg
\author{G.~Plante}\columbia
\author{J.~Qin}\purdue
\author{H.~Qiu}\wis % left Jun 2019
\author{D.~Ram\'irez~Garc\'ia}\freiburg
\author{S.~Reichard}\zurich
\author{A.~Rocchetti}\freiburg
\author{N.~Rupp}\heidelberg
\author{J.~M.~F.~dos~Santos}\coimbra
\author{G.~Sartorelli}\bologna
\author{N.~\v{S}ar\v{c}evi\'c}\freiburg % left Oct 2019
\author{M.~Scheibelhut}\mainz % left Oct 2019
\author{S.~Schindler}\mainz % left Mar 2019
\author{J.~Schreiner}\heidelberg
\author{D.~Schulte}\munster
\author{M.~Schumann}\freiburg
\author{L.~Scotto~Lavina}\paris
\author{M.~Selvi}\bologna
\author{F.~Semeria}\bologna % !!!!!  NEW !!!!!
\author{P.~Shagin}\rice
\author{E.~Shockley}\chicago
\author{M.~Silva}\coimbra
\author{H.~Simgen}\heidelberg
\author{A.~Takeda}\tokyo % !!!!!  NEW JP!!!!!
\author{C.~Therreau}\subatech
\author{D.~Thers}\subatech
\author{F.~Toschi}\freiburg
\author{G.~Trinchero}\torino
\author{C.~Tunnell}\rice
\author{M.~Vargas}\munster
\author{G.~Volta}\zurich
\author{O.~Wack}\heidelberg  % left Mar 2019
\author{H.~Wang}\ucla % left Jul 2019
\author{Y.~Wei}\ucsd
\author{C.~Weinheimer}\munster
\author{M.Weiss~Xu}\wis  % !!!!!  NEW !!!!!
\author{D.~Wenz}\mainz
\author{C.~Wittweg}\munster
\author{J.~Wulf}\zurich % left Mar 2019
\author{Z.~Xu}\columbia  % !!!!!  NEW !!!!!
\author{M.~Yamashita}\tokyo  % !!!!!  NEW JP!!!!!
\author{J.~Ye}\ucsd
\author{G.~Zavattini}\altaffiliation[At ]{INFN, Sez. di Ferrara and Dip. di Fisica e Scienze della Terra, Università di Ferrara, via G. Saragat 1, Edificio C, I-44122 Ferrara (FE), Italy}\bologna   % !!!!!  NEW !!!!!
\author{Y.~Zhang}\columbia
\author{T.~Zhu}\columbia
\author{J.~P.~Zopounidis}\paris


\collaboration{XENON Collaboration}
\email[]{xenon@lngs.infn.it}
\noaffiliation


%\date{\today} 
